slimIoT: Scalable Lightweight Attestation Protocol For the Internet of Things

The Internet of Things (IoT) is increasingly intertwined with critical industrial processes, yet contemporary IoT devices offer limited security features, creating a large new attack surface. Remote attestation is a well-known technique to detect cyber threats by remotely verifying the internal state of a networked embedded device through a trusted entity. Multi-device attestation has received little attention although current single-device approaches show limited scalability in IoT applications. Though recent work has yielded some proposals for scalable attestation, several aspects remain unexplored, and thus more research is required. This paper presents slimIoT, a scalable lightweight attestation protocol that is suitable for all IoT devices. slimIoT depends on an efficient broadcast authentication scheme along with symmetric key cryptography. It is resilient against a strong adversary with physical access to the IoT device. Our protocol is informative in the sense that it identifies the precise status of every device in the network. We implement and evaluate slimIoT considering many factors. On the one hand, our evaluation results show a low overhead in terms of memory footprint and runtime. On the other hand, simulations demonstrate that slimIoT is scalable, robust and highly efficient to be used in static and dynamic networks consisting of thousands of heterogenous IoT devices.

==> sections/app1.tex <==

\label{app:a}
\section{Definitions of Time notation in slimIoT}
\begin{table}
	\centering
	\caption{Time notation in slimIoT}
	\label{table1}
	\begin{tabularx}{\columnwidth}{p{.22\columnwidth}X}

		\toprule
		\multicolumn{2}{l}{Time Parameters}                                                                                                                                   \\ \midrule
		$T_s$                                   & The current time of a node                                                                                                   \\
		
		$i$                                    & Integer indicating the current sub-interval per time period (\textit{epoch})                                                                            \\
		$T_i$                                   & The $i^{th}$ time sub-interval                                                                                                          \\
		$T_{int}$                                 & The duration of a specific time sub-interval  $T_i$                                                                                                 \\
		$d$                                    & Disclosure delay of a key in terms of time sub-intervals or seconds                                                                                                         \\

		\bottomrule
		
	\end{tabularx}
\end{table}


\section{Security Analysis}
\label{secana}
slimIoT is a scalable attestation protocol that allows the trusted network operator, the $verifier$, to label all devices in the swarm as healthy, remotely-compromised, or physically-compromised. The goal of a secure attestation scheme is to distinguish between healthy and compromised devices in a swarm {$S$} , where limited false positive cases are accepted but not vice versa. This is formalized by the following adversarial experiment $ATT_{Adv}^{n, c}(j)$, where $Adv$ interacts with $n$ devices in addition to $verifier$, and compromises up to $c$ devices in $S$ according to the  adversarial model presented in Section \ref{sec:preliminaries}, where $c$ $\leq$ $n -1$. Considering that $Adv$ is computationally bounded to the capabilities of the devices deployed in $S$, $Adv$ interacts with the devices a polynomial  number of times $j$, where $j$ is a security parameter. The $verifier$ verifies the attestation aggregates received from attesting $S$ and outputs a decision as 0 or 1. Denoting the decision made  as $A$, $A$ = 1 means that the attestation routine is finished successfully and all devices are labeled correctly, or $A$ = 0 otherwise. A single false negative case marks the entire attestation scheme as insecure.

Similarly to the definition given by \cite{seda2015},  the formal definition of a secure swarm attestation scheme is illustrated as:
%\theoremstyle{definition} 
\begin{definition}[Secure Swarm Attestation]
	 A swarm attestation scheme is secure if $Pr$[$A$ = 1 | $ATT_{Adv}^{n, c}(j)$ == $A$] is negligible for 0 $<$ $c$ $<$ $n$. 
\end{definition}
According to the above definition, we summarize the security of slimIoT with a proof sketch. 
\newline
\newline
\textbf{Security of slimIoT.}
\begin{theorem}[Security of slimIoT]
	slimIoT is a secure scalable attestation protocol under the following conditions:
	\begin{itemize}
		\item The length of the attestation routine, e.g. \textit{epoch}, does not last longer than $T_{Adv}$. 
		\item The PRNG used to generate new random values and keychains is secure.
		\item The underlying MAC scheme is selective forgery resistant and the aggregation scheme is secure.
		\item The operative devices in a swarm meet the minimum hardware requirements for secure attestation.
	\end{itemize}
\end{theorem}
 \begin{proof}
 	Any device $D_i$ in a swarm $S$ is deployed by a trusted network operator, the $verifier$, in a secure state and initialized with a bunch of secrets stored in a secure and isolated area in the memory that can only be accessed either physically or by the attestation code inside it. The attestation report for any $D_i$ is a binary value set in the $i^{\text{th}}$ position of an $n$-bit vector, dedicated for physical attacks detection, in addition to an attest value verifying the software integrity against remote attacks (if asked).  
 	
 	We distinguish between three different cases for the adversary. We start with the case where $Adv$ is remote. As explained in Section \ref{sec:preliminaries}, $Adv$ can't tamper with the attestation code and secrets according to the rules enforced by the MPU. She is only able to give a proper attestation report for the underlying software-compromised  $D_i$ when being able to break the selective forgery resistance MAC scheme. This can be achieved with a negligible probability due to the selective forgery resistance property. Furthermore, to ensure that this fake attestation report could be accepted by the $verifier$, $Adv$ must aggregate it with all attestation reports from healthy children, and this requires authenticating these reports by getting to know to the group-wide secret values: $K_0$ and $Nonce$. Learning these secrets is not possible without performing a physical attack. 
 	
 	Next, we consider the case where $Adv$ is physically tampering with $D_i$. As this is a time-consuming activity (e.g. it requires at least a few minutes to connect to the device physically, retrieve the stored binary image, and reverse engineer this software, etc.), attesting $S$ is achieved in less time. After missing the first $Nonce_{update}$ broadcast message from the $verifier$, $Adv$ is not able to team up the compromised $D_i$ with $S$ anymore even if she receives all other messages in the successive time periods since authenticating and decrypting these packets depends on the true updated value of $Nonce$ in addition to the correct session key. Therefore, $Adv$ can't send any valid reply and thus by the end of the attestation process, $D_i$ is labeled as physically-compromised. %The probability of labeling $D_i$ as software-compromised is negligible as $Adv$ should not be able to acknowledge receiving the attestation request since this requires breaking the MAC scheme and learning the session encryption key produced, $K_{ENC}$, to decrypt the packets sent in the second time period.
 	
 	The last case is where $Adv$ is more powerful and performs multiple remote and physical attacks at the same time. As a remote attacker, $Adv$ can eavesdrop and record all packets sent between any $D_i$ and the $verifier$ or another $D_j$ during the ongoing attestation process. However, she is still not able to decrypt any encrypted packet as she does not know the current (or even the updated) group-wide secret values. $Adv$ knows only  the first exchanged $N_{new}$ in addition to the exposed session keys. However, by physically attacking other devices and learning old secret values (e.g. $K_0$, $Nonce$), $Adv$ is able to synchronize and know all valid group-wide secrets. This would threaten the security of slimIoT in the future attestation periods if no action is taken. Therefore, in case of detecting a physical attack, the last step of the protocol is updating all group-wide secrets in all healthy devices securely as described in Section \ref{attestphase}. This means that the probability of $Adv$ to get benefits from the exposed group-wide secrets is negligible. Please note that these three cases cover all possibilities of $Adv$ to perform any attack according to the adversarial model presented in Section \ref{sec:preliminaries}.              
 \end{proof}

\section{ A working scenario of slimIoT and its battery impact}
\label{appendix:w}
\begin{figure}[htbp!]
	\centering
	\begin{subfigure}[b]{0.5\textwidth}
		
		\includegraphics[width= \textwidth]{fig/scenario}
		\caption{Working scenario of slimIoT}
		\label{fig:scenario}
	\end{subfigure}
	\begin{subfigure}[b]{0.49\textwidth}
		
		\includegraphics[width= \textwidth]{fig/newFig/power}
		\caption{The impact on battery lifetime} %when running slimIoT on a MicroPnP platform under different rates of time.}
		\label{fig:power}
	\end{subfigure}
	\caption{A working scenario of slimIoT and its battery impact}
	\label{figureapp}
\end{figure}







==> sections/model.tex <==
\section{slimIoT: A Probabilistic Model}
\label{sec:model}

Let $G=(N,L)$ represents a graph for a mesh network where $N$ is the number of IoT devices (vertices) and $L$ is any number of links (edges) that maintains the connectivity between devices. Considering that the network is divided into $M$ non-overlapping clusters, let $C_{i}=\{n_1,n_2,...\} \subseteq N$ be a set of devices representing the $i^{th}$ cluster such that $\bigcap_{j=1}^M C_{j} = \emptyset $. We model the attestation response at iteration $t$ of the $i^{th}$ cluster selected for attestation by 3-tuple $A_{t}^i=\langle C_{i}, S_{t}^i, T_{las} \rangle $, where $S_{t}^i \in \{0,1\}$ as $0$ value indicates that the corresponding cluster has at least one compromised device in this iteration, while $1$ value reflects a safe status. $T_{las}$ is the last time when the cluster has been attested (represented in minutes).

The cluster selection process aims to minimize the communication overhead by attesting the various parts of the network at different time periods while maintaining the security level. However, excluding some clusters from attestation  at iteration $t$ may increase the latency of identifying the remotely-compromised IoT devices in these clusters. Thus, we deal with the communication overhead issue as a trade-off between the cluster selection and the latency of identifying compromised devices, where we leverage the history of every cluster (i.e., $A_{t-1}^i, A_{t-2}^i$, etc. ). More formally, we handle the selection of clusters as a constrained minimization optimization problem objectively defined as: \vspace{-8pt} \begin{equation}
  \begin{aligned}
  & \underset{\alpha_1,\ldots,\alpha_M}{\text{minimize}}\ \sum_{j=1}^{M}  \alpha_j*P(S_{t}^j=1)  
  \ \ \text{s.t. }\
    \frac{\sum_{i=1}^{M} \alpha_{i} * |C_{i}|  }{|N|} \geq Tr_{cov},\\
  & Max\{ (1-\alpha_i)*(T_{now}-A_{t-1}^i.T_{las}) :\ i\in\{1,\dots,M\}\} \leq T_{Max}
  \end{aligned}  
  \end{equation}
   where $\alpha_{\bullet}\in \{0,1\}$ is a free variable corresponding to a cluster, $P(S_{t}^j=1)$ represents the probability of the $j^{th}$ cluster being successfully attested, $Tr_{cov}\in [0,1] $ is a threshold specifying the ratio of devices that will be attested, $T_{now}$ is the current attestation time in minutes, and $T_{Max}\in \mathbb{Z}^+$ is the maximum number of minutes that each cluster can be excluded from the attestation process. The first constraint ($Tr_{cov}$) in the objective function is application dependent and can be tied to the time period of attesting against physical attacks, whereas the second constraint ($T_{Max}$) is added to ensure that all clusters have been attested in a pre-defined maximum time window. In the computation of the probability component stated in the objective function, we first assume that the current state of the cluster is independent from the previous states (i.e. $S_{t-1}^j$ ). Thus,  we adopt the Maximum Likelihood Estimation (MLE) method through leveraging the given information history ($\{ A_{1}^j,\dots, A_{t-1}^j \}$) about the state of the cluster at various attestation iterations. More precisely, we first count the number of times that the cluster has been successfully attested as reported in the cluster's history. Then, the resulted number is divided by the number of times that the cluster has been considered in the attestation process. Formally, the probability component for the $j^{th}$ cluster is computed as follow: 
      \begin{equation}
     P(S_{t}^j=1)=\frac{| \{  A_{i}^j: i\in\{1,...,t-1\},  S_{i}^j=1\}|}{| \{  A_{i}^j: i\in\{1,...,t-1\} \}|}
     \end{equation}
     where $|\bullet|$ represents the set cardinality (length).  
     
     It is clear that the selection of both constraints ($Tr_{cov}$ and $T_{Max}$) depends on the context of the application. However, it is important to mention that setting $Tr_{cov}$ to $1$ means that all clusters must be selected and thus no need to enter in the optimization process. 
   
%   With the definition of the probability component, the ultimate step is finding the optimal values of $\{ \alpha_1,\ldots,\alpha_M\}$; however, there is no closed form solution for such a problem as well as it is NP-complete decision problem. Thus, instead of optimizing the free variables in a random way, different useful heuristic functions could be adopted to get the optimal (or sub-optimal) values. In this paper, we propose   
   
   
   
%   Thus, through using the Bayes' rule, the computation of the cluster probability is defined as: 
%    \begin{equation}
%      P(S_{t}^j=1)= \sum_{s\in\{0,1\}} P(S_{t}^j=1|S_{t-1}^j=s)*P(S_{t-1}^j=s)
%      \end{equation}
%  
%   
%%   adopt the Bayes' rule so that the prior probability, $P(S_{t}^j=1)$, of the $j^{th}$ cluster being successfully attested at iteration $t$ is computed using which is applied on the history information (i.e., number of times successfully attested) of the cluster.  
%     
%%             
%               \begin{equation}
%             P(S^{j}_{t}=1|S_{t-1}^j=s)=\frac{| \{ S_{i}^j: i\in\{1,...,t-1\},  S_{i}^j=s \}|}{|\{ A_{1}^j, ..., A_{t-1}^j  \} |}
%             \end{equation}
%             
             
   
   
